Category-Independent Articulated Object Tracking with Factor Graphs

Robots deployed in human-centric environments may need to manipulate a diverse range of articulated objects, such as doors, dishwashers, and cabinets. Articulated objects often come with unexpected articulation mechanisms that are inconsistent with categorical priors: for example, a drawer might rotate about a hinge joint instead of sliding open. We propose a category-independent framework for predicting the articulation models of unknown objects from sequences of RGB-D images. The prediction is performed by a two-step process: first, a visual perception module tracks object part poses from raw images, and second, a factor graph takes these poses and infers the articulation model including the current configuration between the parts as a 6D twist. We also propose a manipulation-oriented metric to evaluate predicted joint twists in terms of how well a compliant robot controller would be able to manipulate the articulated object given the predicted twist. We demonstrate that our visual perception and factor graph modules outperform baselines on simulated data and show the applicability of our factor graph on real world data.

==> tex/B_vision.tex <==

% \begin{align}
%     \mathcal{L}_{ij}
%         &= (\beta_{ij} - \hat{\beta}_{ij})^2 \\
%         &+ \beta_{ij} \| \bm{c_{ij}} - \bm{\hat{c}_{ij}} \|^2 \\
%         &+ \beta_{ij} \| \bm{t_{ij_v}} - \bm{\hat{t}_{ij_v}} \|^2 \\
%         &+ \beta_{ij} \| \bm{t_{ij_\omega}} - \bm{\hat{t}_{ij_\omega}} \|^2 \\
%         &+ \beta_{ij} \| \lieExp{\bm{t_{ij}}} \bm{c_{ij}} - \lieExp{\bm{\hat{t_{ij}}}} \bm{\hat{c}_{ij}} \|^2 \\
%         &+ \beta_{ij} \| \bm{\sigma}(\bm{\hat{c}_{i-1:i+1,j-1:j+1}}) \|^2 \\
%         &+ \beta_{ij} \| \bm{\sigma}(\bm{\hat{t}_{i-1:i+1,j-1:j+1}}) \|^2 \\
%     \mathcal{L}
%         &= \mathcal{L}_{\beta} + \beta(\gamma_c \mathcal{L}_{c} + \gamma_{\delta_v} \mathcal{L}_{\delta_v} + \gamma_{\delta_\omega} \mathcal{L}_{\delta_\omega} + \gamma_{\tilde{c}} \mathcal{L}_{\tilde{c}} \\
%         &\hspace{47pt}+ \gamma_{\sigma_c} \mathcal{L}_{\sigma_c} + \gamma_{\sigma_\delta} \mathcal{L}_{\sigma_\delta})
% \end{align}

\todo{Copied from Thesis, safe to use?}
For a pixel $i,j$ let us denote the predicted motion features as $\hat{\bm{m\!f}}_{i,j} = (\hat{\beta}_{i,j}, \hat{\bm{c}}_{i,j}, \hat{\bm{t}}_{i,j})$ and the ground truth motion feature map as $\bm{m\!f}_{i,j} = (\beta_{i,j}, \bm{c}_{i,j}, \bm{t}_{i,j})$. We will use a supervised pixel-wise loss as defined through
\begin{align} 	
	\label{eqn:pixel_loss}
	&\mathcal{L}_{\textrm{pixel, super}}
	(
		\bm{m\!f}_{i,j}
		\hat{\bm{m\!f}}_{i,j},
	) \\
	    &\quad= \left( \beta_{i,j} - \hat{\beta}_{i,j} \right)^2 \\
		&\quad\quad + \beta_{i,j}
			\euclideannorm{\bm{c}_{i,j} - \hat{\bm{c}}_{i,j}}^2 \\
		&\quad\quad + \beta_{i,j} \mathcal{L}_{\textrm{transformation}}\left( \bm{t}_{i,j}, \hat{\bm{t}}_{i,j} \right) \\
		&\quad\quad + \beta_{i,j} 
			\euclideannorm{
				\bm{t}_{i,j} \bm{c}_{i,j} 
				- \hat{\bm{t}}_{i,j} \hat{\bm{c}}_{i,j}
			}^2 .
\end{align}
where we scale each euclidean norm additionally with the ground truth importance of that pixel. As a result pixels with low or no importance at all are contributing less to the total loss.

The first term $\left( \beta_{i,j} - \hat{\beta}_{i,j} \right)^2$ in \Cref{eqn:pixel_loss} simply compares the predicted importance to the ground truth importance.

The second term $\beta_{i,j}
\euclideannorm{\bm{c}_{i,j} - \hat{\bm{c}}_{i,j}}^2$ in \Cref{eqn:pixel_loss} will ensure that the predicted part center is close to the ground truth part center.

For the transformation $\bm{t}$ governance in the third term $\beta_{i,j} \mathcal{L}_{\textrm{transformation}}\left( \bm{t}_{i,j}, \hat{\bm{t}}_{i,j} \right)$ in \Cref{eqn:pixel_loss} we have to consider two things. 

First, as we formulated the output of the neural motion feature predictor of the transformation in the log-space of $SE(3)$ (i.e. $se(3)$), we can directly use within a L2-norm: $\euclideannorm{\bm{t}_{i,j}-\hat{\bm{t}}_{i,j}}^2$.

Second, since the rotation is expressed dimensionless and the translation is given in meters, we have to ensure both are on an equal scale. Therefore, we will scale the difference between both transformations by $r$:
\begin{equation}
	\mathcal{L}_{\textrm{transformation}}\left( \bm{t}_{i,j}, \hat{\bm{t}}_{i,j} \right) =
	\euclideannorm{
		r \left( \bm{t}_{i,j} - \hat{\bm{t}}_{i,j} \right)
	}^2
\end{equation}
where $r$ should be in \realspace{6}. In our implementation we have chosen to weight the difference of rotations by 10, resulting in a vector of 
$r = 
\begin{bmatrix}
	1, 1, 1, 10, 10, 10
\end{bmatrix}^T$.

The last term $\beta_{i,j} 
\euclideannorm{
	\bm{T}_{i,j} \bm{c}_{i,j} 
	- \hat{\bm{T}}_{i,j} \hat{\bm{c}}_{i,j}
}^2$ in \Cref{eqn:pixel_loss} first transforms the predicted and ground truth center from the current time step to the next one. We then will compare both transformed centers and they should be close to one another. This can be seen as the process of ensuring that in the next time step both centers end up at the same position. 

In addition to the supervised pixel-loss $\mathcal{L}_{\textrm{pixel, super}}$, we will use an unsupervised variance loss. The main idea is that for pixels that belong to the same part, the predicted center and transformation should be equal in its neighborhood ($3 \times 3$ in our case). For a given pixel $i, j$ the variance for either the center $\sigma_{\bm{c}}$ or the transformation $\sigma_{\bm{t}}$ around this pixel is given through
\begin{align}
	&\mathcal{L}_{\textrm{pixel, variance}}(\hat{\bm{q}}_{i,j}) = 
	\sigma_q \\
	&\quad = 
		\left( \sum_{\tilde{i} = -1}^{1} \sum_{\tilde{j} = -1}^{1} \frac{\hat{q}_{i+\tilde{i}, j+\tilde{j}}^2 }{9} \right) \\
	&\quad\quad - 
		\left( \sum_{\tilde{i} = -1}^{1} \sum_{\tilde{j} = -1}^{1} \frac{\hat{q}_{i+\tilde{i}, j+\tilde{j}}}{9} \right) ^2
\end{align}
where $q \in \left\{\bm{c}, \bm{t} \right\}$. The division by 9 is rooted in our neighborhood size of $3 \times 3 = 9$.

This operation can be efficiently implemented by a sliding window over both spatial dimensions (width and height) of the motion feature map.

The complete loss for a pixel $i,j$ is then given by
\begin{align}
	\label{eqn:full_variance_loss}
	&\mathcal{L}_{\textrm{pixel, full}}
	(
		\bm{m\!f}_{i,j}
		\hat{\bm{m\!f}}_{i,j},
	)\\
	&\quad= 
	\mathcal{L}_{\textrm{pixel, super}}
	(
		\bm{m\!f}_{i,j}
		\hat{\bm{m\!f}}_{i,j},
	)\\
	&\quad\quad+
	\beta_{i,j} 
	\left(
	\mathcal{L}_{\textrm{pixel, variance}}(\hat{\bm{c}_{i,j}})
	\mathcal{L}_{\textrm{pixel, variance}}(\hat{\bm{t}_{i,j}})
	\right)
\end{align}
where, similarly as before, we will scale the variance based on the ground truth importance of the pixel.

Eventually, we calculate the final loss
\begin{equation}
	\mathcal{L}_{\textrm{full}}(\bm{m\!f}, \hat{\bm{m\!f}}) = 
	\sum_{i=1}^{W} \sum_{j=1}^{H}
		\mathcal{L}_{\textrm{pixel, full}}
		(
		\bm{m\!f}_{i,j}
		\hat{\bm{m\!f}}_{i,j}
		)
\end{equation}
by adding up all pixel-wise losses.
